Program Execution on Reconfigurable Multicore Architectures

Based on the two observations that diverse applications perform better on different multicore architectures, and that different phases of an application may have vastly different resource requirements, Pal et al. proposed a novel reconfigurable hardware approach for executing multithreaded programs. Instead of mapping a concurrent program to a fixed architecture, the architecture adaptively reconfigures itself to meet the application's concurrency and communication requirements, yielding significant improvements in performance. Based on our earlier abstract operational framework for multicore execution with hierarchical memory structures, we describe execution of multithreaded programs on reconfigurable architectures that support a variety of clustered configurations. Such reconfiguration may not preserve the semantics of programs due to the possible introduction of race conditions arising from concurrent accesses to shared memory by threads running on the different cores. We present an intuitive partial ordering notion on the cluster configurations, and show that the semantics of multithreaded programs is always preserved for reconfigurations "upward" in that ordering, whereas semantics preservation for arbitrary reconfigurations can be guaranteed for well-synchronised programs. We further show that a simple approximate notion of efficiency of execution on the different configurations can be obtained using the notion of amortised bisimulations, and extend it to dynamic reconfiguration.

==> eptcsdata.tex <==
\providecommand{\firstpage}{83}
\providecommand{\publicationstatus}{D. Orchard and N. Yoshida (Eds.): Programming Language Approaches to \\ Concurrency- and Communication-Centric Software (PLACES 2016).\\
EPTCS 211, 2016, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.211.9}{10.4204/EPTCS.211.9}}

